Performance-Feedback Autoscaling with Budget Constraints for Cloud-based Workloads of Workflows

The growing popularity of workflows in the cloud domain promoted the development of sophisticated autoscaling policies that allow automatic allocation and deallocation of resources. However, many state-of-the-art autoscaling policies for workflows are mostly plan-based or designed for batches (ensembles) of workflows. This reduces their flexibility when dealing with workloads of workflows, as the workloads are often subject to unpredictable resource demand fluctuations. Moreover, autoscaling in clouds almost always imposes budget constraints that should be satisfied. The budget-aware autoscalers for workflows usually require task runtime estimates to be provided beforehand, which is not always possible when dealing with workloads due to their dynamic nature. To address these issues, we propose a novel Performance-Feedback Autoscaler (PFA) that is budget-aware and does not require task runtime estimates for its operation. Instead, it uses the performance-feedback loop that monitors the average throughput on each resource type. We implement PFA in the popular Apache Airflow workflow management system, and compare the performance of our autoscaler with other two state-of-the-art autoscalers, and with the optimal solution obtained with the Mixed Integer Programming approach. Our results show that PFA outperforms other considered online autoscalers, as it effectively minimizes the average job slowdown by up to 47% while still satisfying the budget constraints. Moreover, PFA shows by up to 76% lower average runtime than the competitors.

==> title.tex <==
\begin{titlepage}


\begin{center}

% \topskip0pt
% \vspace*{\fill}

% \textbf{\Large Performance-Feedback Autoscaling} \\
% \vspace{4pt}
% \textbf{\Large with Budget Constraints} \\
% \vspace{4pt}
% \textbf{\Large for Cloud-based Workloads of Workflows}

% \bigskip
% \bigskip

% \textbf{\Large Technical Report} \\

% \bigskip
% \bigskip

% \textit{A short, polished version of this technical report has been submitted for publication\\
% to the IEEE Cluster 2019 conference, and is currently awaiting review}

% \bigskip
% \bigskip


%{\large Authors are anonymized to fulfill the conference requirements}
% {\large Alexey Ilyushkin, Andr\'e Bauer, Alessandro V. Papadopoulos,\\
% Ewa Deelman, Alexandru Iosup}

% Delft University of Technology, the Netherlands,
% University of W\"urzburg, Germany, \\
% M\"alardalen University, Sweden,
% University of Southern California, USA, \\
% Vrije Universiteit Amsterdam, the Netherlands
% a.s.ilyushkin@tudelft.nl, andre.bauer@uni-wuerzburg.de, alessandro.papadopoulos@mdh.se, deelman@isi.edu, a.iosup@vu.nl

\title{Performance-Feedback Autoscaling with Budget Constraints for Workloads of Workflows: Technical Report}

\author[1]{Alexey Ilyushkin}
\author[2]{Andr\'e Bauer}
\author[3]{Alessandro V. Papadopoulos}
\author[4]{Ewa Deelman}
\author[5,1]{Alexandru Iosup}
\affil[1]{Delft University of Technology, the Netherlands}
\affil[2]{University of W\"urzburg, Germany}
\affil[3]{M\"alardalen University, Sweden}
\affil[4]{University of Southern California, USA}
\affil[5]{Vrije Universiteit Amsterdam, the Netherlands}

\maketitle

\bigskip
\bigskip

\vspace*{\fill}
May 23, 2019

\end{center}

\end{titlepage}

